Watch and Learn: Optimizing from Revealed Preferences Feedback

A Stackelberg game is played between a leader and a follower. The leader first chooses an action, then the follower plays his best response. The goal of the leader is to pick the action that will maximize his payoff given the follower's best response. In this paper we present an approach to solving for the leader's optimal strategy in certain Stackelberg games where the follower's utility function (and thus the subsequent best response of the follower) is unknown. Stackelberg games capture, for example, the following interaction between a producer and a consumer. The producer chooses the prices of the goods he produces, and then a consumer chooses to buy a utility maximizing bundle of goods. The goal of the seller here is to set prices to maximize his profit---his revenue, minus the production cost of the purchased bundle. It is quite natural that the seller in this example should not know the buyer's utility function. However, he does have access to revealed preference feedback---he can set prices, and then observe the purchased bundle and his own profit. We give algorithms for efficiently solving, in terms of both computational and query complexity, a broad class of Stackelberg games in which the follower's utility function is unknown, using only "revealed preference" access to it. This class includes in particular the profit maximization problem, as well as the optimal tolling problem in nonatomic congestion games, when the latency functions are unknown. Surprisingly, we are able to solve these problems even though the optimization problems are non-convex in the leader's actions.

==> general-NONOISE-proofs.tex <==
\section{Detailed Analysis of~\Cref{sec:general}}
\label{sec:omitproofs}

Just as in~\Cref{sec:conversion}, we start by considering the
following convex program associated with $\hat x$
\begin{align}
&\max_{x \in \cA_F} \phi(x) \qquad \label{eq:objective}\\ \mbox{ such
that }\qquad &x_j \leq \hat x_j \mbox{ for every }j\in
[d]\label{eq:bound}
\end{align}
%% Since $\phi$ is an increasing function, we know that $\hat x$ is the
%% unique optimal solution of the program.
The Lagrangian of the program
is\[
\cL(x, p) = \phi(x) - \sum_{j = 1}^d p_j (x_j - \hat x_j),
\]
where $p_j$ is the dual variable for each constraint~\eqref{eq:bound}
and the vector $p$ is also interpreted as the action of the
leader. We can interpret the Lagrangian as the payoff function of a
zero-sum game, in which the leader is the minimization player and the
follower is the maximization player. To guarantee the fast convergence of
our later use of gradient descent, we will restrict the leader to play
actions in $\cP$m as defined in~\eqref{eq:P}. It is known that such a
zero-sum game has value $V$: the leader has a minimax strategy $p^*$
such that $\cL(x, p^*) \leq V$ for all $x\in \cA_F$, and the follower
has a maxmin strategy $x^*$ such that $\cL(x^*, p) \geq V$ for all
$p\in \cP$. We first state the following lemma about the \emph{value}
of this zero-sum game.

\begin{lemma}
The value of the Lagrangian zero-sum game is $V = \phi(\hat x)$, that is
\[
\max_{x\in \cA_F} \min_{p\in \cP} \cL(x, p) =  \min_{p\in \cP} \max_{x\in \cA_F} \cL(x, p) = \phi(\hat x)
\]
\end{lemma}
\begin{proof}
The proof is identical to the proof of~\Cref{lem:BPduality}.
\end{proof}

An approximate minimax equilibrium of a zero-sum game is defined as
follows.

\begin{definition}
\label{def:approxeq}
Let $\alpha \geq 0$. A pair of strategies $p\in \cP$ and $x\in \cA_F$
form an $\alpha$-{approximate minimax equilibrium} if
\[
\cL(x, p) \geq \max_{x'\in \cA_F} \cL(x', p) - \alpha \geq V - \alpha \qquad \mbox{ and } \qquad
\cL(x, p) \leq \min_{p'\in \cP} \cL(x, p') + \alpha \leq V + \alpha.
\]
\end{definition}

First observe that fixing a strategy $x$, the maximization player's best response in this zero-sum game
is the same as the follower's best response in the Stackelberg game.

\begin{claim}
Let  $p' \in \cP$ be any action of the leader, then
\[
\arg\max_{x\in \cA_F} \cL(x, p') = x^*(p')
\]
\label{eq:equiv}
\end{claim}

\begin{proof}
We can write
\begin{align*}
\arg\max_{x\in \cA_F} \cL(x, p') &= \arg\max_{x\in \cA_F} \left[\phi(x) - \langle p', x - \hat x\rangle \right]\\
&= \arg\max_{x\in \cA_F}  \left[\phi(x) - \langle p', x \rangle \right]\\
&= \arg\max_{x\in \cA_F}  U_F(p', x)
\end{align*}
The second equality follows from the fact that $\langle p', \hat
x \rangle$ is independent of the choice of $x$.
\end{proof}





Now we show that if a strategy pair $(p', x')$ is an approximate
minimax equilibrium in the zero-sum game, then $p'$ approximately
induces the target action $\hat x$ of the follower. Hence, our task reduces to finding an approximate minimax
equilibrium of the Lagrangian game.
\begin{lemma}
\label{lem:eqclose}
Suppose that a pair of strategies $(p', x')\in \cP\times \cA_F$ forms
an $\alpha$-approximate minimax equilibrium. Then the induced follower
action $x^*(p')$ satisfies $\|\hat x - x^*(p')\| \leq
\sqrt{4\alpha/\sigma}$.
\end{lemma}

\begin{proof}
By the definition of approximate minimax equilibrium, we have
\[
\phi(\hat x) - \alpha \leq \cL(x', p') \leq \phi(\hat x) + \alpha
\]
and also by~\Cref{eq:equiv},
\[
\max_{x\in \cA_F} \cL(x, p') - \alpha = \cL(x^*(p'), p') -\alpha
\leq \cL(x', p') \leq \phi(\hat x) + \alpha
\]

Note that
\[
\cL(\hat x, p') = \phi(\hat x) - \langle p', \hat x - \hat x\rangle = \phi(\hat x).
\]
It follows that $\cL(x^*(p') , p') \leq \cL(\hat x, p') +
2\alpha$. Since $\phi$ is a $\sigma$-strongly concave function, we
know that fixing any leader's action $p$, $\cL$ is also a
$\sigma$-strongly concave function in $x$. By~\Cref{lem:sconvex} and
the above argument, we have
\[
2 \alpha \geq \cL(x^*(p'), p') - \cL(\hat x, p') \geq \frac{\sigma}{2}\|x^*(p') - x\|^2
\]
Hence, we must have $\|x^*(p') - x\| \leq \sqrt{4\alpha/\sigma}$.
\end{proof}

To compute an approximate minimax equilibrium, we will use the
following $T$-round no-regret dynamics: the leader plays online
gradient descent (a ``no-regret'' algorithm), while the follower selects
a best response every round. In particular, the leader will produce a
sequence of actions $\{p^1, \ldots , p^T\}$ against the follower's
best responses $\{x^1, \ldots, x^T\}$ such that for each round $t\in
[T]$:
\[
p^{t+1} = \Pi_\cP\left[ p^t - \eta \cdot \nabla_p \cL(x^t, p^t)\right]
\qquad \mbox{ and }\qquad
x^t = \argmax_{x\in \cA_F} \cL(x, p^t).
\]
At the end of the dynamics, the leader has \emph{regret} defined as
\[
\cR_L \equiv \frac{1}{T} \sum_{t=1}^T \cL(x^t, p^t) - \frac{1}{T} \min_{p\in \cP}\sum_{t=1}^T\cL(x^t, p).
\]


Now take the average actions for both players for this dynamics:
$\overline x = \frac{1}{T} \sum_{t=1}^T x^t$ and $\overline p
= \frac{1}{T} \sum_{t=1}^T p^t$. A well-known result by~\cite{FS96}
shows that the average plays form an approximate minimax equilibrium.

\begin{theorem}[\cite{FS96}]
\label{thm:fs96}
$(\overline p, \overline x)$ forms a $\cR_L$-approximate minimax
equilibrium of the Lagrangian zero-sum game.
\end{theorem}

To simulate the no-regret dynamics, we will have the following
$T$-round dynamics between the leader and the follower: in each round
$t$, the leader plays action $p^t$ based the gradient descent update
and observes the induced action $x^*(p^t)$. The gradient of the
Lagrangian $\nabla_p \cL$ can be easily computed based on the
observations. Recall from~\Cref{eq:equiv} that the follower's best
responses to the leader's actions are the same in both the Stackelberg
game and the Lagrangian zero-sum game. This means that the gradient of
the Lagrangian can be obtained as follows
\[
\nabla_p \cL(x^*(p'), p') = \left( \hat x - x^*(p') \right).
\]

In the end, the algorithm will output the average play of the leader
$1/T\sum_{t=1}^T p^t$. The full description of the algorithm $\LL$ is
presented in~\Cref{alg:learnlead}, and before we present the proof
of~\Cref{thm:generalmain}, we first include the no-regret guarantee of
gradient descent.


\begin{lemma}[\cite{Z03}]\label{lem:gd_regret}
  Let $\cD$ be a closed convex set such that $\|\cD\|\leq D$, and let
  $c^1,\dots,c^T$ be a sequence of differentiable, convex functions
  with bounded gradients, that is for every $x\in \cD$,$ ||\nabla
  c^t(x) ||_2 \leq G$.  Let $\eta = \frac{D}{G\sqrt{T}}$ and
  $\omega^{1} = \proj{\cD} \left[\mathbf{0}\right]$ be arbitrary.
  Then if we compute $\omega^{1},\dots,\omega^{T} \in \cD$ based on
  gradient descent $\omega^{t+1} = \proj{\cD}\left[\omega^t -
    \eta\nabla c(\omega^t)\right] $, the regret satisfies
\begin{equation}
\cR \equiv \frac{1}{T} \sum_{t=1}^T c^t(\omega^{t}) - \min_{\omega \in \cD}
\frac{1}{T}\sum_{t=1}^T c^t(\omega) \leq \frac{G D}{\sqrt{T}}
\label{eq:gd_regret}
\end{equation}
\end{lemma}


\begin{proof}[Proof of~\Cref{thm:generalmain}]
We will first bound the regret of the leader in the no-regret
dynamics. Each vector of $\cP$ has norm bounded by
$\sqrt{d}\lambda_F$. Also, since the gradient of the Lagrangian at
point $p'$ is
\[
\nabla_p \cL(x^*(p'), p') = (\hat x - x^*(p')),
\]
we then know that the gradient is bounded the norm of $\cA_F$, which
is $\gamma$. The regret is bounded by
\[
\cR_L = \frac{\sqrt{2d}\lambda_F \gamma}{\sqrt{T}}.
\]
Let $\overline x = 1/T\sum_{t=1}^T x^*(p^t)$ denote the average play
of the follower. It follows from~\Cref{thm:fs96} that $(\hat
p, \overline x)$ forms an $\cR_L$-approximate minimax equilibrium, and
so by~\Cref{lem:eqclose}, we have
\[
\|\hat x - x^*(\hat p) \| \leq \sqrt{\frac{4\cR_L}{\sigma}} =
\sqrt{\frac{4\sqrt{2d}\lambda_F \gamma}{\sigma\sqrt{T}}}.
\]
Plugging in our choice of $T$, we get $\|x^*(\hat p)
- \hat x\|\leq \eps$, and also the total number of observations on the
follower is also $T$.
\end{proof}

Finally, we give the proof of~\Cref{thm:genmain}.

\begin{proof}[Proof of~\Cref{thm:genmain}]
Since for each $x^t$, the approximate evaluation based on $x^*(p^t)$
satisfies $|\psi(x^t) - \psi(x^*(p^t))| \leq \lambda_L \eps$,
by~\Cref{lem:zero} we know that the action $\hat x$ output by
$\zero(d\eps\lambda_L, \cA_F)$ satisfies
\[
\Expectation \left[\psi(\hat x)\right] \geq \max_{x\in \cA_F}\psi(x) - d\eps\lambda_L
 = \max_{p\in \cA_L} U_L(p, x^*(p)) - d\eps\lambda_L.
\]
Finally, we will use $\LL(\hat x, \eps)$ to output a leader action
$\hat p$ such that $\|x^*(\hat p) - \hat x\| \leq \eps$, and so
$\psi(x^*(\hat p)) \geq \psi(\hat x) - \lambda_L\eps$. Therefore, in
the end we guarantee that
\[
\Expectation\left[U_L(\hat p , x^*(\hat p))\right] = \Expectation\left[\psi(\hat p)\right]
 \geq \Expectation\left[\psi(\hat x) \right]
 -\lambda_L \eps \geq \max_{p\in \cA_L} U_L(p, x^*(p)) -
 (d+1)\eps \lambda_L.
\]
Plugging in our choice of $\eps$, we recover the $\alpha$ accuracy
guarantee. Note that in each iteration, the number of observations on
the follower required by the call of $\LL$ is \[
T' = \frac{32d \lambda_F^2\gamma^2}{\eps^4 \sigma^2}
\]
Therefore the total number of observations our algorithm needs is
bounded by
\[
O\left(T'  \times T \right) = \tilde O\left( \frac{d^{5.5} \lambda_F^2 \gamma^2}{\eps^4\sigma^2} \right)
\]
Again plugging in our value of $\eps$, the bound on the number of
observations needed is \[
\tilde O\left(\frac{d^{9.5} \lambda_F^2 \lambda_L^4\gamma^2}{\alpha^4 \sigma^2}\right).\]
Hiding the constants ($\lambda_F, \lambda_L, \gamma$ and $\sigma$), we
recover the bound above.
\end{proof}


==> general-NONOISE.tex <==
\section{General Framework of Stackelberg Games}
\label{sec:general}
Now that we have worked out a concrete application of our method in
the context of learning to maximize revenue from revealed preferences,
we will abstract our techniques and show how they can be used to solve
a general family of Stackelberg games in which the objective of the
follower is unknown to the leader. 
%Along the way, we will also
%generalize our technique to operate in a setting in which the follower
%responds to the leaders actions by only \emph{approximately}
%maximizing her utility function. We will illustrate the utility of
%this generalization by applying our theorem to a $d$-dimensional
%principal-agent problem, in which the leader only observes stochastic
%feedback.

In our general framework, we consider a \emph{Stackelberg game} that
consists of a \emph{leader} with action set $\cA_L$ and a
\emph{follower} with action set $\cA_F$. Each player has a utility
function $U_L, U_F\colon \cA_L\times\cA_F \to \RR$.  In the
corresponding Stackelberg game, the leader chooses an action $p \in
\cA_L$, and then the follower chooses the best response $x^*(p) =
\argmax_{x\in \cA_F} U_F(p, x)$.

The example of maximizing revenue from revealed preferences is a
special case of this framework.  The producer is the leader and his
action space consists of prices $p$ and the follower is the consumer
and her action space is the bundle $x$ she purchases.  The producer's
utility for a pair $(p, x)$ is his revenue minus the cost of producing
$x$ and the consumer's utility is her value for $x$ minus the price
she pays.

In general, we consider solving the leader's optimization problem---find
$p\in \cA_L$ such that $U_L(p, x^*(p))$ is (approximately)
maximized. Formally, we consider a sub-class of Stackelberg games that have the following structure.

\begin{definition}
\label{def:problem}
An instance is a \emph{Stackelberg game} $\cS(\cA_L, \cA_F, \phi)$ which
consists of two players---the \emph{leader} and the \emph{follower} such that:
\begin{itemize}
\item the leader has action set $\cA_L\subseteq \RR^d$,
the follower has action set $\cA_F\subseteq \RR^d$, both of which are
convex and compact;
\item the follower's utility function $U_F\colon \cA_L\times \cA_F\to \RR$
 takes the form
\[
U_F(p, x) = \phi(x) - \langle p, x\rangle,
\]
where $\phi\colon \RR^d \to \RR$ is a strongly concave, differentiable
function unknown to the leader;
\item the leader's utility function $U_L\colon \cA_L \times \cA_F\to \RR$ is
a possibly unknown function.
\end{itemize}
The optimization problem associated with the game instance is
$\max_{p\in \cA_L} \psi(p, x^*(p))$, where $x^*(p) = \arg\max_{x\in \cA_F}
U_F(p, x)$.
\end{definition}

Our first step to solve the problem is to rewrite the leader's utility
function so that it can be expressed as a function only in the
follower's action. For each action of the follower $x\in \cA_F$, the
set of leader's actions that induce $x$ is
\[
P^*(x) = \{p \in \cA_L\mid x^*(p) = x\}.
\]
Among all of the leader's actions that induce $x$, the optimal one is:
\[
p^*(x) = \argmax_{p\in P^*(x) } U_L(p, x),
\]
where ties are broken arbitrarily.
We can then rewrite the leader's objective as a function of only
$x$:
\begin{equation} \label{eq:psi}
\psi(x) = U_L(p^*(x) , x).
\end{equation}

Note that to approximately solve the leader's optimization problem, it
is sufficient to find the follower's action $\hat x\in \cA_F$ which
approximately optimizes $\psi_F(\cdot)$, together with the action
$\hat p\in \cA_L$ that approximately induces $\hat x$. Before we
present the algorithm, we state the assumptions on the utility
functions of the two players that we will need.
\begin{assumption}
\label{ass:general}
The game $\cS(\cA_L, \cA_F, \phi)$ satisfies the following properties.
\begin{enumerate}
\item The function $\psi\colon \cA_L \to \RR$ defined in~\eqref{eq:psi} is concave and $\lambda_L$-Lipschitz;
\item The function $\phi\colon \cA_F \to \RR$ is non-decreasing, $\sigma$-strongly concave and $\lambda_F$-Lipschitz;
% \item The action space of the follower $\cA_F$ is well-rounded and has bounded norm $\|\cA_F\| \leq \gamma$;
\item The action space of the leader $\cA_L$ contains the following set
\begin{equation}
\cP = \{p\in \RRP^d \mid \|p\| \leq \sqrt{d} \lambda_F\};
\label{eq:P}
\end{equation}
\ju{Hard to keep track of $\cP$ vs. $\cP(x)$.}\ar{Agreed.}\ar{Why does
  the ball need to be origin centered? In the pricing example we
  needed the feasible region to contain $0$ so that we could argue
  that the profit maximizing prices were the gradient of the valuation
  function, but that was specific to the revealed preferences
  setting. Also its not really a ball if it is centered at the origin,
  but contains only non-negative points.}\sw{fixed; switched to $P^*$ now}
\item The action space of the follower $\cA_F$ has bounded diameter, $\|\cA_F\| \leq \gamma$.
\end{enumerate}

\end{assumption}






\subsection{Inducing a Target Action of the Follower}
\label{sec:generalinduce}
We first consider the following sub-problem.  Given a target action
$\hat x$ of the follower we want to learn an action $\hat p$ for the leader such that the
induced action satisfies
\[
\| x^*(\hat p) - \hat x\| \leq \eps.
\]
We now give an algorithm to learn $\hat p$ that requires only
polynomially many observations of the follower's action.



\iffalse %%% MOVED TO APPENDIX
Moreover, learning $\hat p$ should require only polynomially many observations of the follower's action.

Just as in~\Cref{sec:conversion}, we consider the following convex program associated with $\hat x$
\begin{align}
&\max_{x \in \cA_F} \phi(x) \qquad \label{eq:objective}\\ \mbox{ such
that }\qquad &x_j \leq \hat x_j \mbox{ for every }j\in
[d]\label{eq:bound}
\end{align}
%% Since $\phi$ is an increasing function, we know that $\hat x$ is the
%% unique optimal solution of the program.
The Lagrangian of the program
is\[
\cL(x, p) = \phi(x) - \sum_{j = 1}^d p_j (x_j - \hat x_j),
\]
where $p_j$ is the dual variable for each constraint~\eqref{eq:bound}
and the vector $p$ is also interpreted as the action of the
leader. We can interpret the Lagrangian as the payoff function of a
zero-sum game, in which the leader is the minimization player and the
follower is the maximization player. To guarantee the fast convergence of
our later use of gradient descent, we will restrict the leader to play
actions in $\cP$m as defined in~\eqref{eq:P}. It is known that such a
zero-sum game has value $V$: the leader has a minimax strategy $p^*$
such that $\cL(x, p^*) \leq V$ for all $x\in \cA_F$, and the follower
has a maxmin strategy $x^*$ such that $\cL(x^*, p) \geq V$ for all
$p\in \cP$. We first state the following lemma about the \emph{value}
of this zero-sum game.
\sw{decide to use the zero-sum game
language here, so we can also talk about the extension of the follower
only approximately best responds. also adds some variety to the
analysis. but please make sure this is not getting readers confused}

\begin{lemma}
The value of the Lagrangian zero-sum game is $V = \phi(\hat x)$, that is
\[
\max_{x\in \cA_F} \min_{p\in \cP} \cL(x, p) =  \min_{p\in \cP} \max_{x\in \cA_F} \cL(x, p) = \phi(\hat x)
\]
\end{lemma}
\begin{proof}
The proof is identical to the proof of~\Cref{lem:BPduality}.
\end{proof}

An approximate minimax equilibrium of a zero-sum game is defined as
follows.

\begin{definition}
\label{def:approxeq}
Let $\alpha \geq 0$. A pair of strategies $p\in \cP$ and $x\in \cA_F$
form an $\alpha$-{approximate minimax equilibrium} if
\[
\cL(x, p) \geq \max_{x'\in \cA_F} \cL(x', p) - \alpha \geq V - \alpha \qquad \mbox{ and } \qquad
\cL(x, p) \leq \min_{p'\in \cP} \cL(x, p') + \alpha \leq V + \alpha.
\]
\end{definition}

First observe that fixing a strategy $x$, the maximization player's best response in this zero-sum game
is the same as the follower's best response in the Stackelberg game.

\begin{claim}
Let  $p' \in \cP$ be any action of the leader, then
\[
\arg\max_{x\in \cA_F} \cL(x, p') = x^*(p')
\]
\label{eq:equiv}
\end{claim}

\begin{proof}
We can write
\begin{align*}
\arg\max_{x\in \cA_F} \cL(x, p') &= \arg\max_{x\in \cA_F} \left[\phi(x) - \langle p', x - \hat x\rangle \right]\\
&= \arg\max_{x\in \cA_F}  \left[\phi(x) - \langle p', x \rangle \right]\\
&= \arg\max_{x\in \cA_F}  U_F(p', x)
\end{align*}
The second equality follows from the fact that $\langle p', \hat
x \rangle$ is independent of the choice of $x$.
\end{proof}





Now we show that if a strategy pair $(p', x')$ is an approximate
minimax equilibrium in the zero-sum game, then $p'$ approximately
induces the target action $\hat x$ of the follower. Hence, our task reduces to finding an approximate minimax
equilibrium of the Lagrangian game.
\begin{lemma}
\label{lem:eqclose}
Suppose that a pair of strategies $(p', x')\in \cP\times \cA_F$ forms
an $\alpha$-approximate minimax equilibrium. Then the induced follower
action $x^*(p')$ satisfies $\|\hat x - x^*(p')\| \leq
\sqrt{4\alpha/\sigma}$.
\end{lemma}

\begin{proof}
By the definition of approximate minimax equilibrium, we have
\[
\phi(\hat x) - \alpha \leq \cL(x', p') \leq \phi(\hat x) + \alpha
\]
and also by~\Cref{eq:equiv},
\[
\max_{x\in \cA_F} \cL(x, p') - \alpha = \cL(x^*(p'), p') -\alpha
\leq \cL(x', p') \leq \phi(\hat x) + \alpha
\]

Note that
\[
\cL(\hat x, p') = \phi(\hat x) - \langle p', \hat x - \hat x\rangle = \phi(\hat x).
\]
It follows that $\cL(x^*(p') , p') \leq \cL(\hat x, p') +
2\alpha$. Since $\phi$ is a $\sigma$-strongly concave function, we
know that fixing any leader's action $p$, $\cL$ is also a
$\sigma$-strongly concave function in $x$. By~\Cref{lem:sconvex} and
the above argument, we have
\[
2 \alpha \geq \cL(x^*(p'), p') - \cL(\hat x, p') \geq \frac{\sigma}{2}\|x^*(p') - x\|^2
\]
Hence, we must have $\|x^*(p') - x\| \leq \sqrt{4\alpha/\sigma}$.
\end{proof}

To compute an approximate minimax equilibrium, we will use the
following $T$-round no-regret dynamics: the leader plays online
gradient descent (a ``no-regret'' algorithm), while the follower selects
a best response every round. In particular, the leader will produce a
sequence of actions $\{p^1, \ldots , p^T\}$ against the follower's
best responses $\{x^1, \ldots, x^T\}$ such that for each round $t\in
[T]$:
\[
p^{t+1} = \Pi_\cP\left[ p^t - \eta \cdot \nabla_p \cL(x^t, p^t)\right]
\qquad \mbox{ and }\qquad
x^t = \argmax_{x\in \cA_F} \cL(x, p^t).
\]
At the end of the dynamics, the leader has \emph{regret} defined as
\[
\cR_L \equiv \frac{1}{T} \sum_{t=1}^T \cL(x^t, p^t) - \frac{1}{T} \min_{p\in \cP}\sum_{t=1}^T\cL(x^t, p).
\]


Now take the average actions for both players for this dynamics:
$\overline x = \frac{1}{T} \sum_{t=1}^T x^t$ and $\overline p
= \frac{1}{T} \sum_{t=1}^T p^t$. A well-known result by~\cite{FS96}
shows that the average plays form an approximate minimax equilibrium.

\begin{theorem}[\cite{FS96}]
\label{thm:fs96}
$(\overline p, \overline x)$ forms a $\cR_L$-approximate minimax
equilibrium of the Lagrangian zero-sum game.
\end{theorem}

To simulate the no-regret dynamics, we will have the following
$T$-round dynamics between the leader and the follower: in each round
$t$, the leader plays action $p^t$ based the gradient descent update
and observes the induced action $x^*(p^t)$. The gradient of the
Lagrangian $\nabla_p \cL$ can be easily computed based on the
observations. Recall from~\Cref{eq:equiv} that the follower's best
responses to the leader's actions are the same in both the Stackelberg
game and the Lagrangian zero-sum game. This means that the gradient of
the Lagrangian can be obtained as follows
\[
\nabla_p \cL(x^*(p'), p') = \left( \hat x - x^*(p') \right).
\]
In the end, the algorithm will output the average play of the leader
$1/T\sum_{t=1}^T p^t$. The full description of the algorithm $\LL$ is
presented in~\Cref{alg:learnlead}, and the formal guarantee is the
following.
\fi
\begin{algorithm}[h]
  \caption{Learning the leader's action to induce a target follower's action: $\LL(\hat x, \eps)$}
 \label{alg:learnlead}
  \begin{algorithmic}
    \STATE{\textbf{Input:} A target follower action $\hat x\in \cA_F$, and target accuracy $\eps$}
    \INDSTATE{Initialize:
 restricted action space $\cP=\{p\in  \RR_+^{d} \mid \|p\|\leq \sqrt{d}\lambda_F\}$
      \[
      p^1_j = 0 \mbox{ for all }j \in [d] \qquad
      T= \frac{32d \lambda_F^2\gamma^2}{\eps^4 \sigma^2} \qquad
\eta= \frac{\sqrt{2}\gamma}{\sqrt{d}\lambda_F\sqrt{T}}
      \]
    }
    \INDSTATE{For $t = 1, \ldots , T$:}
    \INDSTATE[2]{Observe the induced action by the follower $x^*(p^t)$}
    \INDSTATE[2]{Update leader's action:
      \[
      \tilde{p}^{t+1}_j = p^t_j - \eta \left(\hat x_j - x^*(p^t)_j\right) \mbox{ for each }j\in [d],\qquad
p^{t+1} = \proj{\cP} \left[\hat p^{t+1}\right]
      \]
}
    \INDSTATE{\textbf{Output:} $\hat p = 1/T\sum_{t=1}^T p^t.$}
    \end{algorithmic}
  \end{algorithm}


\begin{theorem}
\label{thm:generalmain}
Let $\hat x \in \cA_F$ be a target follower action and $\eps >
0$. Then $\LL(\hat x, \eps)$ outputs a leader action $\hat p$ such
that the induced follower action satisfies $\|\hat x - x^*(\hat
p)\|\leq \eps$ and the number of observations it needs is no more
than \[T=O \left(\frac{d \lambda_F^2\gamma^2}{\eps^4 \sigma^2}\right)\]
\end{theorem}


\iffalse %% MOVED TO APPENDIX
\begin{proof}
We will first bound the regret of the leader in the no-regret
dynamics. Each vector of $\cP$ has norm bounded by
$\sqrt{d}\lambda_F$. Also, since the gradient of the Lagrangian at
point $p'$ is
\[
\nabla_p \cL(x^*(p'), p') = (\hat x - x^*(p')),
\]
we then know that the gradient is bounded the norm of $\cA_F$, which
is $\gamma$. The regret is bounded by
\[
\cR_L = \frac{\sqrt{d}\lambda_F \gamma}{\sqrt{T}}.
\]
Let $\overline x = 1/T\sum_{t=1}^T x^*(p^t)$ denote the average play
of the follower. It follows from~\Cref{thm:fs96} that $(\hat
p, \overline x)$ forms an $\cR_L$-approximate minimax equilibrium, and
so by~\Cref{lem:eqclose}, we have
\[
\|\hat x - x^*(\hat p) \| \leq \sqrt{\frac{4\cR_L}{\sigma}} = \sqrt{\frac{4\sqrt{d}\lambda_F \gamma}{\sigma\sqrt{T}}}.
\]
Plugging in our choice of $T$, we get $\|x^*(\hat p)
- \hat x\|\leq \eps$, and also the total number of observations on the
follower is also $T$.
\end{proof}
\fi



\subsection{Optimizing Leader's Utility}
Now that we know how to approximately induce any action of the
follower using $\LL$, we are ready to give an algorithm to optimize the
leader's utility function $U_L$. Recall that we can write the $U_L$ as
a function $\psi$ that depends only of the follower's action. $\psi$ requires that to obtain utility $\psi(x)$, the leader must play the \emph{optimal} action $p$ that induces the follower to play $x$.

\begin{assumption}
\label{ass:consistent}
For any $\hat x\in \cA_F$ and $\eps > 0$, the instantiation $\LL(\hat
x, \eps)$ returns $\hat p$ such that
\[
\hat p = p^*\left(x^*(\hat p)\right).
\]
\end{assumption}
Whenever this assumption holds, we can use $\LL$ to allow the leader to obtain utility $U_L(\hat p , x^*(\hat
p)) = \psi(x^*(\hat p))$.

While~\Cref{ass:consistent} appears to be quite strong, we can often achieve it. Recall that we were able to satisfy~\Cref{ass:consistent} in our revealed preferences application by operating in the interior of the feasible region of the follower's action space, and we can similarly do this in our principal-agent example. Moreover, it is trivially satisfied whenever the leader's objective function \emph{depends only on the follower's action}, since in this case, every leader-action $p$ which induces a particular follower-action $x$ is optimal. This is the case, for example, in our routing games application in~\Cref{sec:flow}.

Now we will show how to use the algorithm $\zero$ to find an
approximate optimal point for the function $\psi$. First, we will use
$\LL$ to provide approximate function evaluation for $\psi$ at each
$\hat x\in \cA_F$: our algorithm first runs $\LL(\hat x, \eps)$ to
learn a price vector $\hat p$, and we will use the observed function
value on the induced follower action $\psi(x^*(\hat p))$ as an
approximation for $\psi(\hat x)$. Since $\LL$ guarantees that
$\|x^*(\hat p) - \hat x\| \leq \eps$, by the Lipschitz property of
$\psi$ we have
\[
|\psi(\hat x) - \psi(x^*(\hat p))| \leq \lambda_L \eps.
\]
With these approximate evaluations, $\zero$ can then find a
$(d\lambda_L \eps)$-approximate optimizer of
$\psi$ with only $\tilde O(d^{4.5})$ iterations by~\Cref{lem:zero}.
The full algorithm is presented in~\Cref{alg:lopt}.

\begin{algorithm}[h]
  \caption{Leader learn to optimize: $\lop(\cA_F, \alpha)$}
 \label{alg:lopt}
  \begin{algorithmic}

    \STATE{\textbf{Input:} Follower action space $C$, and target
    accuracy $\alpha$} \INDSTATE{Initialize: number of iterations
    $T= \tilde O(n^{4.5})$ and $\eps = \frac{\alpha}{ \lambda_L (d +
    1)}$}
    \INDSTATE{For $t = 1, \ldots , T$:}
    \INDSTATE[2]{$\zero(d\eps\lambda_L, \cA_F)$ queries the objective value for action $x^t\in \cA_F$}
    \INDSTATE[2]{Let $ p^t = \LL(x^t, \eps)$ and observe the induced action $x^*( p^t)$}
    \INDSTATE[2]{Send $\psi(x^*(p^t))$ to $\zero(d\eps\lambda_L, C_\delta)$ as an approximate evaluation of $\psi(x^t$)}
    \INDSTATE{$\hat x = \zero(d\eps\lambda_L, \cA_F)$}
    \INDSTATE{$\hat p = \LL(\hat x, \eps)$}
    \INDSTATE{\textbf{Output:} the leader action $\hat p$}
    \end{algorithmic}
  \end{algorithm}


\begin{theorem}
\label{thm:genmain}
Let $\alpha > 0$ be the target accuracy. The instantiation
$\lop(\cA_F, \alpha)$ computes a leader action $\hat p$ along with its
induced follower action $x^*(\hat p)$ that satisfies
\[\Expectation[
U_L(\hat p, x^*(\hat p))] \geq \max_{p\in \cA_L} U_L(p, x^*(p)) - \alpha,
\] and the number of observations the algorithm requires of the follower is bounded by
\[
\tilde O\left(  \frac{d^{9.5}}{\alpha^4}\right).
\]
\end{theorem}

\iffalse %MOVED TO APPENDIX
\begin{proof}
Since for each $x^t$, the approximate evaluation based on $x^*(p^t)$
satisfies $|\psi(x^t) - \psi(x^*(p^t))| \leq \lambda_L \eps$,
by~\Cref{lem:zero} we know that the action $\hat x$ output by
$\zero(d\eps\lambda_L, \cA_F)$ satisfies
\[
\Expectation \left[\psi(\hat x)\right] \geq \max_{x\in \cA_F}\psi(x) - d\eps\lambda_L
 = \max_{p\in \cA_L} U_L(p, x^*(p)) - d\eps\lambda_L.
\]
Finally, we will use $\LL(\hat x, \eps)$ to output a leader action
$\hat p$ such that $\|x^*(\hat p) - \hat x\| \leq \eps$, and so
$\psi(x^*(\hat p)) \geq \psi(\hat x) - \lambda_L\eps$. Therefore, in
the end we guarantee that
\[
\Expectation\left[U_L(\hat p , x^*(\hat p))\right] = \Expectation\left[\psi(\hat p)\right]
 \geq \Expectation\left[\psi(\hat x) \right]
 -\lambda_L \eps \geq \max_{p\in \cA_L} U_L(p, x^*(p)) -
 (d+1)\eps \lambda_L.
\]
Plugging in our choice of $\eps$, we recover the $\alpha$ accuracy
guarantee. Note that in each iteration, the number of observations on
the follower required by the call of $\LL$ is \[
T' = \frac{16d \lambda_F^2\gamma^2}{\eps^4 \sigma^2}
\]
Therefore the total number of observations our algorithm needs is
bounded by
\[
T' \times (T + 1) = \tilde O\left( \frac{d^{5.5} \lambda_F^2 \gamma^2}{\eps^4\sigma^2} \right)
\]
Again plugging in our value of $\eps$, the bound on the number of
observations needed is \[
\tilde O\left(\frac{d^{9.5} \lambda_F^2 \lambda_L^4\gamma^2}{\alpha^4 \sigma^2}\right).\]
Hiding the constants ($\lambda_F, \lambda_L, \gamma$ and $\sigma$), we
recover the bound above.
\end{proof}
\fi



==> routingexample.tex <==
\section{A Routing Game Where Social Cost is Not Convex in The Tolls}
\label{sec:routingexample}

As we stated in the introduction, we can give a simple example of a
routing game in which the function mapping a set of tolls on each of
the edges to the social cost of the equilibrium routing in the routing
game induced by those tolls is not a convex function of the tolls.
The example is related to the canonical examples of \emph{Braess'
Paradox} in routing games.

\usetikzlibrary{positioning}
\definecolor{processblue}{cmyk}{0.96,0,0,0}

\begin{figure}[h!]
\begin{center}
\begin{tikzpicture}[-latex ,auto ,node distance = 2 cm and 4cm ,on grid ,
thick ,
state/.style ={ circle ,top color =white , bottom color = processblue!20 ,
draw,processblue , text=blue , minimum width =1 cm}]
\node[state] (S) {$S$};
\node[state] (A) [above right =of S] {$A$};
\node[state] (T) [below right=of A] {$T$};
\node[state] (B) [below right =of S] {$B$};
\path (S) edge [bend left = 15] node[above left] {$4x/10$} (A);
\path (S) edge [bend right = 15] node[below left] {$1/2$} (B);
\path (B) edge [bend right = 15] node[below right] {$4x/10$} (T);
\path (A) edge [bend left = 15] node[above right] {$1/2$} (T);
\path (A) edge [bend right = 25] node[left] {$1/200 + \tau_{1}$} (B);
\path (A) edge [bend left = 25] node[right] {$\tau_2$} (B);
\end{tikzpicture}
\end{center}
\caption{\footnotesize{A routing game in which the function mapping tolls to social cost of the unique equilibrium routing is not convex.  In this example, there are $n$ players each trying to route $1/n$ units of flow from $S$ to $T$.  There are two edges from $A$ to $B$ with tolls $\tau_1$ and $\tau_2$, and we assume without loss of generality that all other tolls are fixed to $0$.  Each edge is labeled with the latency function indicating the cost of using that edge when the congestion on that edge is $x \in [0,1]$.  Note that the latencies (excluding the tolls) on every edge are bounded in $[0,1]$.}}
\end{figure}

Let $\mathit{SC}(\tau_1,\tau_2)$ be the function that maps a pair of tolls for the two $A \rightarrow B$ edges to the social cost (excluding the tolls) of the equilibrium routing.  For each of the inputs we consider, the equilibrium will be unique, so multiplicity of equilibria is irrelevant.

First, consider the set of tolls $\tau = \tau_1 = \tau_2 = 0$.  It is not hard to verify that the unique equilibrium is for every player to use the route $S \rightarrow A \rightarrow B \rightarrow T$ using the $A \rightarrow B$ edge on the right (with latency $0$).\footnote{Since the graph is a DAG, we can use backwards induction.  From $A$, it can never cost more to go $A \rightarrow B \rightarrow T$ than to go $A \rightarrow T$.  Since one can go from $A$ to $B$ for a cost of $0$, players are indifferent about ending up at node $A$ and node $B$.  Since $S \rightarrow A$ can never cost more than $S \rightarrow B$, and players are indifferent between $A$ and $B$, every player would choose the path $S \rightarrow A \rightarrow B \rightarrow T$ (using the $0$ latency path from $A$ to $B$.}  Each player will experience a total latency of $1$ along their route.  Thus $\mathit{SC}(\tau) = 8n/10$.

Now consider the tolls $\tau'$ in which $\tau_1 = 1, \tau_2 = 2$.  At these tolls, it is not hard to verify that the unique equilibrium is for $n/2$ players to use $S \rightarrow A \rightarrow T$ and half to use $S \rightarrow B \rightarrow T$.\footnote{At these tolls, no player will never use either $A \rightarrow B$ edge.  Thus, they will balance the traffic so that $S \rightarrow A \rightarrow T$ and $S \rightarrow B \rightarrow T$ have equal cost.  By symmetry, half will go through $A$ and half through $B$.}  Every player experiences a total latency of $2/10 + 1/2 = 7/10$.  Thus $\mathit{SC}(t') = 7n/10$.

Finally, consider the convex combination $99\tau/100 + \tau'/100$ in which $\tau_1 = 1/100$ and $\tau_2 = 1/50$.  In this case, the unique equilibrium routing will have every player use the route $S \rightarrow A \rightarrow B \rightarrow T$ but using the $A \rightarrow B$ edge on the left (with latency $1/200$ and latency-plus-toll $3/200$).  To see why, observe that if a player were at $A$, then no matter what the other players are doing, the cheapest path to $T$ is to go $A \rightarrow B \rightarrow T$ using the left edge (note that the right edge has latency-plus-toll $1/50$ whereas the left edge has latency-plus-toll $3/200$).  Thus, the cost of going $B \rightarrow T$ is exactly $1/2$ and the cost of going $A \rightarrow B \rightarrow T$ is exactly $1/2 + 3/200$.  Now, if the player is at $S$, going $S \rightarrow B \rightarrow T$ costs exactly $1$, whereas going $S \rightarrow A \rightarrow B \rightarrow T$ costs \emph{at most} $4/10 + 1/2 + 3/200 = 183/200 < 1/2.$  Thus, every player will choose the path $S \rightarrow A \rightarrow B \rightarrow T$, using the left $A \rightarrow B$ edge.  Every player experiences a total latency of exactly $183/200$.  Thus, $\mathit{SC}(t'') = 183n/200$.

But, since
\begin{align*}
\mathit{SC}(99\tau/100 + \tau'/100)
={} &\frac{183n}{200} \\
>{} &\frac{99}{100} \cdot \frac{8n}{10} + \frac{1}{100} \cdot \frac{7n}{10} \\
={} &\frac{99}{100} \cdot \mathit{SC}(\tau) + \frac{1}{100} \cdot \mathit{SC}(\tau'),
\end{align*}
we can see that the function $\mathit{SC}(\tau)$ is not convex in $\tau$.

==> target.tex <==
\subsection{Enforcing a Target Flow via Tolls}
In this section, we show how to adaptively learn a set of edge tolls
to enforce a target flow as Wardrop equilibrium. Tolls are additional
costs on the edges charged on the players using the edge. Given a toll
vector $\tau = (\tau_e)_{e\in E}\in \RR_+^{m}$, we could define a new
latency function on each edge: $\ell_e^\tau(f_e) = \ell(f_e) +
\tau_e$, which gives rise to a different routing game.

\sw{we still hope for some assumption that allows latency function
  like $x^2$}
\paragraph{Assumption}{ 
For each latency function $\ell_e$, there exists a constant $\sigma >
0$ such that $\ell_e(x) \geq \sigma x$ for all $0\leq x\leq 1$.
Recall that the potential function $\Phi(x)$ is a function on $m$
variables $(x_e)_{e\in E}$, and the Hessian $\partial^2 \Phi$ at each
$x$ is a diagonal matrix with entries $\frac{\partial \ell_e}{\partial
  x_e} \geq \sigma$. Therefore, we know that $\partial^2 \Phi \succeq
\sigma I$, and so the $\Phi$ is a $\sigma$-strongly convex function.}




\paragraph{Model}{
Given a target flow $g\in \cF$, we want to find a vector of edge tolls
$\tau$ such that the induced Wardrop equilibrium flow of the game
$\cG(G, \ell^\tau, \cD)$
\[\cE(\tau) =  \arg\min_{f\in \cF} \sum_e \int_0^{f_e} \ell_e^\tau(x) dx
\footnote{The resulting equilibrium is unique because the potential
  function is strictly convex ($\ell_e$ is strictly increasing).}\]
satisfies $\|\cE(\tau) - g\|_2 \leq \delta$ for some small
$\delta > 0$. In our settings, the latency functions $\ell_e$ are
unknown to the algorithm, but we have access to an \emph{equilibrium
  oracle} that takes a toll vector $\tau$ as input and returns an
equilibrium flow $\cE(\tau)$. Our goal is to approximately induce the
target flow $g$ while minimizing the number of queries to the oracle.}







Before we present the algorithm, we first include a result
from~\citet{FJM04}, which gives the existence of a toll vector to
enforce any target flow in $\cF$ exactly.

\begin{lemma}[\citet{FJM04}]
  \label{lem:existoll}
Let $g$ be any flow in $\cF$, then there exists a set of tolls $\tau$
over the edges such that $\cE(\tau) = g$. 
\end{lemma}


To compute such set of edge tolls, we consider the following
convex program adapted from~\Cref{nash-flow}:
\begin{align}
&\min_{f} \, \Phi(f)\\ \mbox{s.t. }&\quad f_e = \sum_i f_e^i \leq g_e
\quad &\mbox{ for all }e \in
  E\label{eq:target}\\ &\quad f^i\in \cF_i \quad &\mbox{ for all }
  i\in [n]
\end{align}

\iffalse
The central authority can use edge tolls to induce certain target flow
$g$. Given a vector of tolls $\tau = (\tau_e)_e \in \RR^E_+$ on the
network edges, the latency function on each edge $e$ becomes
$\ell_e^\tau (x)\coloneqq \ell_e(x) + \tau_e$, and so the delay of an
agent who chooses path $P$ is now $\ell_P(f) + \tau(P)$, where
$\tau(P)\coloneqq \sum_{e\in P} \tau_e$. The new potential function
induced by the a toll vector $\tau$ is
\[
\Phi'(f) = \sum_e \int_0^{f_e} [\ell_e(f_e) ]
\]
\fi

We will work with the Lagrangian of the convex program extensively. For each
constraint~\ref{eq:target}, we introduce a dual variable $\tau_e$,
which we will interpret as the toll on that edge:
\begin{align*}
%% \max_{\tau} \min_{f\in F}
\cL(f, \tau) = \sum_e \left[\int_0^{f_e} \ell_e(x)\, dx +
  \tau_e(f_e - g_e)  \right]
\end{align*}

We could write down the Lagrangian dual objective function as well:
\[
h(\tau) = \min_{f\in \cF} \cL(f, \tau) = \min_{f\in \cF} \left[ \sum_e
  \left(\int_0^{f_e} \ell_e(x)\, dx + \tau_e(f_e - g_e) \right)\right]
\]
\iffalse
Since the target flow $g$ is a strictly feasible solution to the
convex program, the \emph{Slater's condition} holds, so we have strong
duality:\fi
We will first show that strong duality holds.
\begin{lemma}
\[\max_{\tau\in \RR_+^{m}} \min_{f\in \cF} \cL(f, \tau) = \min_{f\in \cF}\max_{\tau\in \RR_+^{m}}  \cL(f, \tau)  = \Phi(g)\]
\end{lemma}

\begin{proof}
First, it is easy to see that 
\[\max_{\tau\in \RR_+^{m}} \min_{f\in \cF} \cL(f, \tau) \leq \min_{f\in \cF}\max_{\tau\in \RR_+^{m}}  \cL(f, \tau).\]
We can now lower bound the left hand side by $\Phi(g)$. By~\Cref{lem:existoll}, we
know there exists a toll vector $\tau^*\in \RR_+^{m}$ such that $\cE(\tau^*) = g$.
\begin{align*}
\max_{\tau\in \RR_+^{m}} \min_{f\in \cF} \cL(f, \tau) &\geq
\min_{f\in \cF} \cL(f, \tau^*)\\
 &= \min_{f\in \cF} \sum_e
\left[\int_0^{f_e} \ell_e(x)\, dx + \tau^*_e(f_e - g_e) \right]\\
&=\min_{f\in \cF} \sum_e \left[\int_0^{f_e} \left(\ell_e(x) + \tau^*_e \right)\, dx -
  \tau^*_e g_e  \right]\\
&=\min_{f\in \cF} \sum_e \left[\int_0^{f_e} \left(\ell_e^{\tau^*}(x) \right)\, dx  \right]
- \sum_e \tau_e^* g_e\\
&= \sum_e \left[\int_0^{g_e} \left(\ell_e^{\tau^*}(x) \right)\, dx  \right]
- \sum_e \tau_e^* g_e\\
&= \sum_e \left[\int_0^{g_e} \left(\ell_e(x) \right)\, dx  \right] = \Phi(g)
\end{align*}
Next we will upper bound the right hand side by $\Phi(g)$. 
\begin{align*}
  \min_{f\in \cF}\max_{\tau\in \RR_+^{m}}  \cL(f, \tau)& \leq \max_{\tau\in \RR_+^{m}}  \cL(g, \tau)\\
  & = \max_{\tau\in \RR_+^{m}}\sum_e \left[\int_0^{g_e} \left(\ell_e(x) \right)\, dx + \tau_e(g_e-g_e)  \right]\\
  & = \Phi(g)
\end{align*}
Therefore, we have shown that
\[\max_{\tau\in \RR_+^{m}} \min_{f\in \cF} \cL(f, \tau) = \min_{f\in \cF}\max_{\tau\in \RR_+^{m}}  \cL(f, \tau)  = \Phi(g)\]
\end{proof}



\subsection{Zero-Sum Game between Tolls and Flows}
We will interpret the Lagrangian objective as the payoff function of a
zero-sum game between the flow player $f$ (minimizing $\cL$) and the
toll player $\tau$ (maximizing $\cL$). We first derive that the
equilibrium of the game corresponds to our target flow and toll.

\begin{lemma}\label{lem:eq-target}
  Suppose $(f^*, \tau^*)$ is an equilibrium of the game that achieves
  \[
   \argmax_{\tau\in\RR_+^{m}}\min_{f\in \cF} \cL(f, \tau).
  \]
  Then $f^* = g$, and the toll vector $\tau^*$ enforces the target flow $g$, i.e. $\cE(\tau^*) = g$.
\end{lemma}

\begin{proof}
Let $f\in \cF$ such that $f\neq g$. Since both $f$ and $g$ route the
same amount of flow for all pairs of source and destination, we know
there exists an edge $e\in E$ such that $f_e > g_e$. Then we could
find a toll vector $\tau'$ with a sufficiently large coordinate
$\tau'_e$ such that $\cL(f, \tau') > \Phi(g)$. Therefore, any flow
$f\neq g$ will have $\max_{\tau\in \RR_+^{m}} \cL(f, \tau) >
\Phi(g)$, so we must have $f^* = g$.

Note that $g$ is a best response to $\tau^*$, so we have
\begin{align*}
g &= \argmin_{f\in \cF} \cL(f, \tau^*)\\ 
&=\argmin_{f\in \cF} \sum_e \left[\int_0^{f_e} \ell_e(x)\, dx +
  \tau^*_e(f_e - g_e)  \right]\\
&=\argmin_{f\in \cF} \sum_e \left[\int_0^{f_e} \left(\ell_e(x) + \tau^*_e \right)\, dx -
  \tau^*_e g_e  \right]\\
&=\argmin_{f\in \cF} \sum_e \left[\int_0^{f_e} \left(\ell_e(x) + \tau^*_e \right)\, dx  \right]
\end{align*}
Therefore, $\cE(\tau^*) = g$.
\end{proof}

We now focus on a \emph{restricted} version of the game, in which the
toll player has a bounded action space $\Lambda$. We show that if the
restricted action space is sufficiently large, the equilibrium of the
game remains the target flow and toll.

%% For computational reason, we need to decide a bounded action space
%% $\Lambda$ for the toll player that contains our target toll vector.
%% We assume the set of toll vectors to be $\Lambda = \{\tau \mid 0\leq
%% \tau_e\leq B \}$, and first derive how large $B$ needs to be in order
%% to induce our target flow.

\begin{lemma}
Suppose that we restrict the action space of the toll player to be
$\Lambda=\{\tau\in \RR_+^{m}\mid \|\tau\|_2\leq 2m\}$. Then there is a toll vector $\tau^\bullet\in \Lambda$
such that $(g, \tau^\bullet)$ is an equilibrium of the restricted game
and $g = \cE(\tau^\bullet)$.
\end{lemma}

\begin{proof}
%% By \Cref{lem:eq-target}, we know that $(g, \lambda^*)$ is an equilibrium
%% of the Lagrangian game with value $\Phi(g)$. This means, $g$ gets
%% value at most $\Phi(g)$ no matter what the toll player's strategy in
%% $\Lambda$ is. Now we show that restricting the toll player's action
%% space to $\Lambda$ leaves the value of the game at $\Phi(g)$.

Consider any flow $f\in \cF$ such that $f\neq g$. We want to show that
$\max_{\tau\in \Lambda}\cL(f, \tau) > \max_{\tau_\in \Lambda} \cL(g,
\tau) = \Phi(g)$. Since $f$ and $g$ direct the same amount of flow for
all pairs of source and destination, there exists an edge $\hat e$
such that $f_{\hat e} > g_{\hat e}$. Let $f_{\hat e} - g_{\hat e} =
\delta$. Note that flow $g$ needs to direct an extra amount of
$\delta$ flow through the other edges, and in the worst case the extra
flow will go through all the other edges, so we can bound
\[\sum_{e' \in E\mbox{ s.t. } g_{e'} > f_{e'}} g_{e'} - f_{e'} \leq m\delta.\] Let
\begin{align*}
  \Delta &= \max_\tau \cL(f, \tau) - \max_\tau \cL(g, \tau)\\
&= \max_\tau \left[\Phi(f) - \langle \tau , f-g\rangle \right] - \max_\tau \left[\Phi(g) - \langle \tau , g-g\rangle \right]\\
  &=\left(\Phi(f) - \Phi(g) \right) + \max_\tau \langle \tau , f - g \rangle. 
\end{align*}
Furthermore, we can write 
\begin{align*}
\Phi(f) - \Phi(g) &= \sum_e \left( \int_0^{f_e} \ell_e(x)\,dx - 
  \int_0^{g_e} \ell_e(x)\, dx \right) \\
 &\geq - \sum_{e\in E\mbox{ s.t. } g_e > f_e} \int_{f_e}^{g_e} \ell_e(x)\, dx\\
 &\geq - \sum_{e\in E\mbox{ s.t. } g_e > f_e} \ell_e(g_e)\left(g_e - f_e \right)\\
 &\geq - \left(\max_e \ell_e(g_e)\right) \cdot m\delta
\end{align*}

We can construct a toll vector $\tau'\in \Lambda$ such that
\[
\tau'_e = \begin{cases} 2m &\mbox{ if } f_e > g_e \\
0 &\mbox{ otherwise }
\end{cases}
\]
Then
\[
\max_{\tau\in \Lambda} \langle \tau, f-g \rangle \geq \langle \tau', f - g\rangle \geq 2m\delta
\]
It follows that $\Delta \geq 2m\delta - (\max_e \ell_e(g_e))\cdot
m\delta \geq m\delta > 0$, and so the minmax strategy of restricted
game is $g$.

Now, since both the flow and toll player play in compact sets $\cF$
and $\Lambda$, the minimax theorem~\citep{Kneser52} shows that there
exists an equilibrium $(g, \tau^{\bullet})$. Similar
to~\Cref{lem:eq-target}, we know that $g$ is a best response to
$\tau^{\bullet}$, and so $\cE(\tau^\bullet) = g$.
\end{proof}

\iffalse
\begin{lemma}
  There exists some toll vector $\tau^*\in \Lambda$ such that $g =
  \cE(\tau)$ as long as $B \geq m \cdot \left(\max_e \ell(g_e)
  \right)$.
\end{lemma}


\begin{proof}


Let $f\in \cF$ be a flow such that $f \neq g$ and
\[
\Delta = \max_\tau \cL(f, \tau) - \max_\tau \cL(g, \tau) =
\left(\Phi(f) - \Phi(g) \right) + \max_\tau \langle \tau , f - g \rangle. 
\]
Let $f'$ be a flow such that $f_e = \min\{f_e, g_e\}$ for all $e\in E$.
  Note that flows $(f - f')$ and $(g - f')$ are ``disjoint'',
i.e.\ there is no edge such that they both have positive flows on. It
follows that the toll player's best response against flow $f$ is to
set tolls to be $1$ on the edges with positive flows in $(f-g')$.
\[
\max_\tau \langle \tau, f - g\rangle = \max_\tau \langle \tau, (f - h)
+(h - g)\rangle = B \cdot \|f - h\|_1.
\]

Furthermore, we can write 
\begin{align*}
\Phi(f) - \Phi(g) &= \sum_e \left( \int_0^{f_e} \ell_e(x)\,dx - 
  \int_0^{g_e} \ell_e(x)\, dx \right) \\
 &\geq - \sum_e \int_{h_e}^{g_e} \ell_e(x)\, dx\\
 &\geq - \sum_e \ell_e(g_e) (g_e - h_e) \geq  - \left( \max_e
   \ell_e(g_e)\right) \cdot \|g - h\|_1
\end{align*}

We know that $(f - h)$ and $(g - h)$ direct the same amount of flows
for all pairs of source and sink. The ratio between their $\ell_1$
norm can be bounded by the length of the longest path, which in turn
can be bounded by number of edges $m$, so 
\[
\|f - h \|_1 \geq \| g - h\|_1 / m.
\]
Finally, we have 
\[
\Delta \geq  B \cdot \|g - h\|_1 / m  - \left(
  \max_e\ell_e(g_e)\right) \cdot \|g - h\|_1.
\]
The right hand side is non-negative as long as $B \geq m \cdot
\left(\max_e \ell(g_e) \right)$.

\end{proof}




Let $\cL(f, \tau) = \sum_e \int_0^{f_e} \ell_e(x)\,dx + \tau_e(f_e -
g_e)$. We can phrase this problem as a zero-sum game between the flow
player (min) and the toll player (max), with the payoff defined by
$\cL(f, \tau)$. Let the value of the game be $\OPT$. Note that $\cL$
can be re-written as
\[
\cL(f, \tau) = \sum_e \left[ \int_0^{f_e} \left(\ell_e(x) +
    \tau_e\right)\, dx  - \tau_e g_e\right],
\]
 and we assume that we have access to an oracle that, given a toll vector $\tau$, returns
an equilibrium flow, i.e.\  
\[
\hat f = \arg\min_{f\in F} \sum_e \int_0^{f_e} (\ell_e(x) + \tau_e)
\, dx, \sw{it is unique?}
\]
which can be thought of as the best response from the flow player
against the tolls. Simultaneously, we have the toll player an
no-regret algorithm, so the empirical play of both players will
converge to an approximate equilibrium of the aforementioned zero-sum
game.


In particular, we will use online gradient descent algorithm, which gives
the following guarantee
\[
R(GD) =\max_{\tau\in D} \frac{1}{T} \sum_{t=1}^T u_t(\tau)-
\frac{1}{T} \sum_{t=1}^T u_t(\tau^t) \leq \frac{D_2 G_2}{\sqrt{T}},
\]
where $G_2$ is a bound on the $\ell_2$ norm of the gradient of all
$u_t$, and $D_2$ is a bound on the $\ell_2$ norm of the toll vectors
in $D$. Also, note that the flow player playing best response for all
rounds has 0 regret. The utility function at each time step $t$ is
simply $u_t(\tau) = \sum_e \tau_e(f_e^t - g_e) = \langle \tau ,
f^t-g\rangle$.\footnote{This is essentially just a function of the
  $\tau$, since $f^t$ is just the best response flow determined by
  $\tau$.}

\fi

Now we present our algorithm in~\Cref{alg:learntoll}. 


\begin{algorithm}[h]
  \caption{Learning Tolls to Enforce Target Flow} \label{alg:learntoll}
  \begin{algorithmic}
    \STATE{\textbf{Input:} A target flow $g\in \cF$, an equilibrium
      oracle $\cE$, action space for tolls $\Lambda=\{\tau\in
      \RR_+^{m}\mid \|\tau\|_2\leq 2m\}$}
    \INDSTATE{Initialize
      \[
      \tau^1_e = 0 \mbox{ for all }e\in E \qquad T = \frac{16m^3}{\delta^4\sigma^2} \qquad \eta = \frac{2m^{3/2}}{\sqrt{T}}
      \]
    }
    \INDSTATE{For $t = 1, \ldots , T$:}
    \INDSTATE[2]{Observe equilibrium flow $\cE(\tau^t)$}
    \INDSTATE[2]{Update toll vector with projected subgradient descent
      \[
      \hat{\tau}^{t+1}_e = \tau^t_e + \eta \left(\cE(\tau^t)_e - g_e
      \right) \mbox{ for each }e\in E,\qquad \tau^{t+1} = \Pi_{\Lambda} \left[\hat\tau^{t+1}\right]
      \]
}
    \INDSTATE{\textbf{Output:} $\hat\tau = 1/T\sum_{t=1}^T \tau^t.$}
    \end{algorithmic}
  \end{algorithm}

\sw{somehow tempted to name this algorithm \sf{LOL}}

\begin{theorem}
For any target flow $g\in \cF$, \Cref{alg:learntoll} that
$\delta$-approximately enforce flow $g$ with at most
$\frac{16m^3}{\delta^4\sigma^2}$ many queries to the equilibrium
oracle.
\end{theorem}

%% Our proof will rely on the following basic fact about strongly convex
%% function.



\begin{proof}
Let $\alpha = \delta^2\sigma/2$. Consider the Lagrangian dual
objective function $h$. We know that any subgradient of $h$ satisfies
$\left(\cE(\tau) - g \right)_{e\in E} \in [-1, 1]^m$, so $h$ is a
$\sqrt{m}$-Lipschitz function. 
%% Since for every toll vector $\tau$, we could observe the equilibrium
%% flow $\cE(\tau)$, which gives a subgradient of the Lagrangian dual
%% objective function $\left(\cE(\tau) - g  \right)_{e\in E} \in [-1, 1]^m$. 
Note that $h$ is a concave function of $\tau$ (so $-h$ is convex), we
could use the projected subgradient descent algorithm to compute an
approximate maxmin strategy $\hat \tau$ for the toll player, i.e.
\[
h(\tau^\bullet) - \alpha \leq h(\hat \tau) \leq h(\tau^\bullet)
\]
By~\Cref{thm:gd}, we need $T = \frac{(2m)^2(m)}{\alpha^2} =
4m^3/\alpha^2$ many queries.

Let $f = \cE(\hat \tau)$, we have $h(\hat \tau) = \cL(f,
\hat\tau)$. We also have $h(\tau^\bullet) = \cL(g, \tau^\bullet) =
\Phi(g) = \cL(g, \hat\tau)$.  It follows that
\[
\cL(g, \hat \tau) - \alpha \leq \cL(f, \hat \tau) \leq  \cL(g, \hat \tau)
\]
Since that $\Phi(\cdot)$ is a $\sigma$-strongly convex function,
$\cL(\cdot, \hat\tau)$ is a $\sigma$-strongly convex function. It
follows from~\Cref{f:sconvex} that $\|f - g\|^2\leq 2\alpha/\sigma =
\delta^2$.
\end{proof}



\iffalse
\begin{lemma}
Suppose that $\hat \tau$ is an $\alpha$-approximate max-min strategy
for the toll player, and let $\hat f = \arg\min_f \cL(f, \hat \tau)$.
Then $\| \hat f - g\| \leq $
\end{lemma}

\begin{proof}
Since $\hat \tau$ is an $\alpha$-approximate max-min strategy, we have
\[
\OPT \leq \cL(\hat f, \hat \tau) \leq \OPT + \alpha.
\]
We also know that $\cL(g, \hat \tau) = \OPT$, as $g$ satisfies all
constraints, and so $|\cL(g, \hat \tau) - \cL(\hat f, \hat \tau) |
\leq \alpha$. \sw{now use our assumption properly.}
\end{proof}


\subsection{Enforcing Approximately Optimal Flow}
\sw{might require a $O(m^4)$ algorithm to transform the dual action
  space into a well-rounded one}

\sw{compose our algorithm with a zeroth-order optimization algorithm}
\fi

